Teach Harder, Learn Poorer: Rethinking Hard Sample Distillation for GNN-to-MLP Knowledge Distillation

To bridge the gaps between powerful Graph Neural Networks (GNNs) and lightweight Multi-Layer Perceptron (MLPs), GNN-to-MLP Knowledge Distillation (KD) proposes to distill knowledge from a well-trained teacher GNN into a student MLP. In this paper, we revisit the knowledge samples (nodes) in teacher GNNs from the perspective of hardness, and identify that hard sample distillation may be a major performance bottleneck of existing graph KD algorithms. The GNN-to-MLP KD involves two different types of hardness, one student-free knowledge hardness describing the inherent complexity of GNN knowledge, and the other student-dependent distillation hardness describing the difficulty of teacher-to-student distillation. However, most of the existing work focuses on only one of these aspects or regards them as one thing. This paper proposes a simple yet effective Hardness-aware GNN-to-MLP Distillation (HGMD) framework, which decouples the two hardnesses and estimates them using a non-parametric approach. Finally, two hardness-aware distillation schemes (i.e., HGMD-weight and HGMD-mixup) are further proposed to distill hardness-aware knowledge from teacher GNNs into the corresponding nodes of student MLPs. As non-parametric distillation, HGMD does not involve any additional learnable parameters beyond the student MLPs, but it still outperforms most of the state-of-the-art competitors. HGMD-mixup improves over the vanilla MLPs by 12.95% and outperforms its teacher GNNs by 2.48% averaged over seven real-world datasets.

==> table_A4.tex <==
\begin{table}[!tbp]
\begin{center}
\caption{A comparison of training time (ms / epoch).}
\label{tab:A4}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccccc}

\toprule
Method & \texttt{Cora} & \texttt{Citeseer} & \texttt{Pubmed} & \texttt{Photo} & \texttt{CS} & \texttt{Physics} \\ \midrule
GLNN & 3.35 & 3.70 & 3.90 & 4.72 & 18.03 & 34.16 \\
KRD & 3.94 & 4.71 & 6.45 & 7.65 & 23.74 & 43.15 \\
HGMD-mixup & 3.71 & 4.33 & 5.74 & 6.86 & 21.75 & 39.51 \\ \bottomrule
    
\end{tabular}} \vspace{-1em}
\end{center}
\end{table}
